Leveraging Experience in Lazy Search

Lazy graph search algorithms are efficient at solving motion planning problems where edge evaluation is the computational bottleneck. These algorithms work by lazily computing the shortest potentially feasible path, evaluating edges along that path, and repeating until a feasible path is found. The order in which edges are selected is critical to minimizing the total number of edge evaluations: a good edge selector chooses edges that are not only likely to be invalid, but also eliminates future paths from consideration. We wish to learn such a selector by leveraging prior experience. We formulate this problem as a Markov Decision Process (MDP) on the state of the search problem. While solving this large MDP is generally intractable, we show that we can compute oracular selectors that can solve the MDP during training. With access to such oracles, we use imitation learning to find effective policies. If new search problems are sufficiently similar to problems solved during training, the learned policy will choose a good edge evaluation ordering and solve the motion planning problem quickly. We evaluate our algorithms on a wide range of 2D and 7D problems and show that the learned selector outperforms baseline commonly used heuristics.

==> inputs/research_questions.tex <==
\section{Research Questions}

\scnote{Now that we have this framework, we can begin to ask some questions.

\begin{enumerate}
    \item[Q1.] Let's consider the case where the model is unknown, we have no side information. What is the optimal policy?

    We can apply an OFU algorithm as done in PAC-MDP algorithms. We define a surrogate MDP where all unknown edges are feasible. We solve for the greedy policy on this MDP and execute it. If we encounter a state not on the MDP, we update it and repeat. 
    
    This algorithm is in fact LazySP. We can bound its performance.
    
    \item[Q2.] Let's consider that we define a prior over MDPs (let's say Bernoulli). What is the optimal Bayesian exploration policy?
    
    Let's say we use a classical BRL algorithm like Bayesian Exploration Bonus (Kolter). I conjecture that would likely involve checking edges on the expected shortest path (plus some bonus for reducing uncertainty). This might lead to a nice anytime behavior.
    
    Another alternate is Osband's Thompson sampling style of algorithms. Sample a MDP, solve the shortest path, check edges, repeat. 
    
    \item[Q3.] Let's now say we have some side information (like an image / a floor plan). We also have a distribution over MDPs (this can be a dataset of worlds). Let's say we want to learn $Q(s,a)$ (this will be in expectation over the worlds). How do we do it?
    
    It seems the problem here is learning a low dimensional representation. It seems the learning community deals with this problem using VAE. If our graph was fixed, we too could train a CVAE. The target input would be the original graph. The conditioning would be edges that are evaluated already. 
    
    Another thing to look at would be graph kernels. 
    
    \item[Q4]. Can we leverage imitation learning of oracles? 
    
    It's trivial to compute a near-optimal policy if the MDP is known (setcover).
\end{enumerate}
}



